DaliID: Distortion-Adaptive Learned Invariance for Identification Models

In unconstrained scenarios, face recognition and person re-identification are subject to distortions such as motion blur, atmospheric turbulence, or upsampling artifacts. To improve robustness in these scenarios, we propose a methodology called Distortion-Adaptive Learned Invariance for Identification (DaliID) models. We contend that distortion augmentations, which degrade image quality, can be successfully leveraged to a greater degree than has been shown in the literature. Aided by an adaptive weighting schedule, a novel distortion augmentation is applied at severe levels during training. This training strategy increases feature-level invariance to distortions and decreases domain shift to unconstrained scenarios. At inference, we use a magnitude-weighted fusion of features from parallel models to retain robustness across the range of images. DaliID models achieve state-of-the-art (SOTA) for both face recognition and person re-identification on seven benchmark datasets, including IJB-S, TinyFace, DeepChange, and MSMT17. Additionally, we provide recaptured evaluation data at a distance of 750+ meters and further validate on real long-distance face imagery.

==> tables/domain.tex <==
\begin{table}[h]
    \centering
    \footnotesize
  \begin{tabular}{p{16mm}|c c c c}
     & None & Moderate & Aggressive & \textbf{Combined} \\
    \hline
    \textit{Low domain shift} & \xmark & \moderate & \cmark & \cmark \\
    \textit{Clean feature space} & \cmark & \moderate & \xmark & \cmark \\  
    
    \end{tabular}
    % \vspace{-2em}
    \caption{Model properties under increasing distortion training. Columns are rows show desirable model properties. Increasing the level of distortion training. By combining multiple feature spaces at inference time, we can get the best of both.}
    \label{tab:my_label}
\end{table}

==> tables/face_ablation.tex <==
\begin{table}
    \footnotesize
    \centering
    \begin{tabular}{ l | c c c}
    \hline\hline
    Setup &  IJB-C & CFP-LD & TinyFace \\
    \hline
    Clean  & 97.38 & & 72.18 \\
    Moderate Distortion Aug& 97.19 & &  \\
    Severe Distortion Aug& 96.91 &  & 74.11 \\
    Severe Distortion-Adaptive & 96.92 & 74.22 \\
    DaliFace & 97.40 & & 73.98 \\
     \hline\hline
     % \multicolumn{4}{l}{AW=adaptive weighting}
    \end{tabular}
    \vspace{-10pt}
    \caption{Ablation study on Face Recognition Datasets. Three settings are represented: standard quality (IJB-C), low resolution (TinyFace), and atmospheric turbulence (CFP-T). It can be seen that DaliFace is the only model that does trade-off accuracy.}
    \label{tab:face_ablation}
\end{table}

==> tables/high-qual-face-tab.tex <==
\begin{table*}[!h]
\centering
\scriptsize
%\begin{tabularx}{\textwidth}{@{}l*{8}{C}c@{}}
\begin{tabular}{|l|c|c|ccccc|c|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}{*}{Venue}} & \multicolumn{1}{c|}{\multirow{2}{*}{Train Data}} &\multicolumn{6}{c|}{High Quality}     & \multicolumn{2}{c|}{Mixed Quality}  \\ \cline{4-11} 
\multicolumn{1}{|c|}{}     & &     & \multicolumn{1}{l|}{\scalebox{0.85}{LFW~\cite{lfw}}}   & \multicolumn{1}{l|}{\scalebox{0.85}{CFP-FP~\cite{cfpfp}}} & \multicolumn{1}{l|}{\scalebox{0.85}{CPLFW~\cite{cplfw}}} & \multicolumn{1}{l|}{\scalebox{0.85}{AgeDB~\cite{agedb}}} & \multicolumn{1}{l|}{\scalebox{0.85}{CALFW~\cite{calfw}}} & \multicolumn{1}{c|}{AVG} & \multicolumn{1}{c|}{IJB-B~\cite{ijbb}} & \multicolumn{1}{c|}{IJB-C~\cite{ijbc}} \\ \hline
CosFace ($m=0.35$)~\cite{wang2018cosface} & CVPR18 &  MS1MV2 & $99.81$ & $98.12$    & $92.28$   & $98.11$   & $95.76$   & $96.82$ & $94.80$   & $96.37$   \\
ArcFace ($m=0.50$)~\cite{deng2019arcface} & CVPR19 &     MS1MV2 & $99.83$ & $98.27$    & $92.08$   & $98.28$   & $95.45$   & $96.78$ & $94.25$   & $96.03$   \\
AFRN~\cite{kang2019attentional} & ICCV19  &  MS1MV2 & $99.85$ & $95.56$    & $93.48$   & $95.35$   & $96.30$   & $96.11$ & $88.50$   & $93.00$   \\
MV-Softmax~\cite{wang2020mis} & AAAI20  &  MS1MV2 & $99.80$ & $98.28$    & $92.83$   & $97.95$   & $96.10$   & $96.99$ & $93.60$   & $95.20$   \\
CurricularFace~\cite{huang2020curricularface} & CVPR20 &   MS1MV2  & $99.80$ & $98.37$    & $93.13$   & $98.32$   & $96.20$   & $97.16$ & $94.80$   & $96.10$   \\
URL~\cite{shi2020towards} &CVPR20 & MS1MV2 & $99.78$ & $98.64$ & - & - & - & - & - & $96.60$ \\
BroadFace~\cite{kim2020broadface} & ECCV20  &  MS1MV2 & $99.85$ & $98.63$ & $93.17$ & $98.38$ & $96.20$ & $97.25$ & $94.97$ & $96.38$ \\

MagFace~\cite{meng2021magface} & CVPR21 &  MS1MV2 & $99.83$ & $98.46$ & $92.87$ & $98.17$ & $96.15$ & $97.10$ & $94.51$ & $95.97$  \\ 
SCF-ArcFace~\cite{li2021spherical} & CVPR21 &  MS1MV2 & $99.82$ & $98.40$    & $93.16$   & $98.30$   & $96.12$   & $97.16$ & $94.74$   & $96.09$  \\ 
DAM-CurricularFace~\cite{liu2021dam} & ICCV21 &  MS1MV2 & - & -  & -  & -   & - & - & $95.12$    & $96.20$ \\ \hdashline
\textbf{AdaFace ($m=0.4$)}  &   CVPR22    & MS1MV2     & $99.82$ & $98.49$    & $93.53$   & $98.05$   & $96.08$   & $97.19$ & $95.67$   & $96.89$  
  \\ \hline \hline
VPL-ArcFace~\cite{deng2021variational} & CVPR21 & MS1MV3 & $99.83$ & $99.11$ & $93.45$ & $98.60$ & $96.12$ & $97.42$ & $95.56$ & $96.76$  \\ \hdashline
\textbf{AdaFace ($m=0.4$)}  &  CVPR22 &  MS1MV3 & $99.83$ & $99.03$ & $93.93$ & $98.17$ & $96.02$ & $97.40$ & $95.84$ & $97.09$  \\ \hline \hline
ArcFace*~\cite{deng2019arcface}& CVPR19 & \scalebox{0.85}{WebFace4M} & $99.83$ & $99.19$ & $94.35$ & $97.95$ & $96.00$ & $97.46$ & $95.75$ & $97.16$ \\ \hdashline
\textbf{AdaFace ($m=0.4$)}     & CVPR22 &     \scalebox{0.85}{WebFace4M}  & $99.80$ & $99.17$ & $94.63$ & $97.90$ & $96.05$ & $97.51$ & $96.03$ & $97.39$  \\ \hline
\end{tabular}

==> tables/scratch.tex <==
\begin{table*}
\scriptsize
\scalebox{0.993}{
\begin{tabular}{l|c|ccc|ccc|ccc|cc}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Method}} & \multicolumn{1}{c|}{\multirow{3}{*}{Train Data}}  &\multicolumn{11}{c|}{Low Quality (IJB-S~\cite{ijbs} and TinyFace~\cite{tinyface})}  \\ 
\cline{3-13}   &    & \multicolumn{3}{c|}{Surveillance-to-Single~\cite{ijbs}}     & \multicolumn{3}{c|}{Surveillance-to-Booking~\cite{ijbs}}    & \multicolumn{3}{c|}{Surveillance-to-Surveillance~\cite{ijbs}}  & \multicolumn{2}{c|}{TinyFace~\cite{tinyface}}   \\
  &  & \multicolumn{1}{c}{Rank-$1$} & \multicolumn{1}{c}{Rank-$5$} & \multicolumn{1}{c|}{$1\%$} & \multicolumn{1}{c}{Rank-$1$} & \multicolumn{1}{c}{Rank-$5$} & \multicolumn{1}{c|}{$1\%$} & \multicolumn{1}{c}{Rank-$1$} & \multicolumn{1}{c}{Rank-$5$} & \multicolumn{1}{c|}{$1\%$} & \multicolumn{1}{c}{Rank-$1$} & \multicolumn{1}{c|}{Rank-$5$} \\ \hline
PFE~\cite{shi2019probabilistic}\scalebox{0.875}{\textcolor{white}{aaa}}  & MS1Mv2~\cite{deng2019arcface}   & $50.16$ & $58.33$  & $31.88$ & $53.60$ & $61.75$    & $35.99$ & $9.20$  & $20.82$   & $0.84$  & -  & -    \\
ArcFace~\cite{deng2019arcface}  & MS1Mv2~\cite{deng2019arcface}   & $57.35$ & $64.42$  & $41.85$ & $57.36$ & $64.95$    & $41.23$ & -    & - & -     & - & -   \\
URL~\cite{shi2020towards}   & MS1Mv2~\cite{deng2019arcface}   & $59.79$ & $65.78$  & $41.06$ & $61.98$ & $67.12$    & $42.73$ & -    & - & -    & $63.89$ &  $68.67$   \\
CurricularFace*~\cite{huang2020curricularface}  & MS1Mv2~\cite{deng2019arcface}   & $62.43$ & $68.68$  & $47.68$ & $63.81$ & $69.74$    & $47.57$ & $19.54$ & $32.80$   & $2.53$     & $63.68$ & $67.65$ \\
AdaFace   & MS1Mv2~\cite{deng2019arcface}   & $65.26$ & $70.53$  & $51.66$ & $66.27$ & $71.61$    & $50.87$ & $23.74$ & $37.47$   & $2.50$    &  $68.21$ & $71.54$   \\ \hline \hline
ArcFace*~\cite{deng2019arcface} & \scalebox{0.86}{WF4M~\cite{webface}}     & $69.26$ & $74.31$ & $57.06$ & $70.31$ & $75.15$ & $56.89$ & $32.13$ & $46.67$ & $5.32$  &  $71.11$  &  $74.38$\\
AdaFace~\cite{Kim_2022_CVPR} &  \scalebox{0.86}{WF4M~\cite{webface}}  &  $70.42$ & $75.29$ & $58.27$ & $70.93$ & $76.11$ & $58.02$ & $35.05$ & $48.22$ & $4.96$  &  $72.02$  &  $74.52$\\
\textbf{DaliFace (ours)} & \\
\hline

\hline
ArcFace*~\cite{deng2019arcface} & \scalebox{0.86}{WF12M~\cite{webface}}     & $69.26$ & $74.31$ & $57.06$ & $70.31$ & $75.15$ & $56.89$ & $32.13$ & $46.67$ & $5.32$  &  $71.11$  &  $74.38$\\
AdaFace~\cite{Kim_2022_CVPR} &  \scalebox{0.86}{WF12M~\cite{webface}}  &  $70.42$ & $75.29$ & $58.27$ & $70.93$ & $76.11$ & $58.02$ & $35.05$ & $48.22$ & $4.96$  &  $72.02$  &  $74.52$\\
\textbf{DaliFace (ours)} \\
\hline
\end{tabular}
}

==> tbspace.tex <==
\makeatletter

%\setlength\belowcaptionskip{5pt \@plus 4pt \@minus 0pt}
%\setlength\abovecaptionskip{9pt \@plus 2pt \@minus 0pt}

% \long\def\@makecaption#1#2{
% \vspace*{\abovecaptionskip}
%    \setbox\@tempboxa\hbox{\small \noindent {\bf #1.}~{\it #2}}
%    \setlength{\@ctmp}{\hsize}
%    \addtolength{\@ctmp}{-\@figindent}\addtolength{\@ctmp}{-\@figindent}
%    % IF longer than one indented paragraph line
%    \ifdim \wd\@tempboxa >\@ctmp
%       % THEN DON'T set as an indented paragraph
%       {\small{\bf #1.}{~\it#2}\par}
%    \else
%       % ELSE center
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
%   \fi\vspace*{\belowcaptionskip}}


\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-1.2ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-.6ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
	                           {\normalfont\large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-.5ex\@plus -.2ex \@minus -.2ex}%
                                     {.2ex \@plus .2ex}%
                                     {\normalfont\large\bfseries}}


\abovedisplayskip=8pt plus 4pt minus 0pt 
\abovedisplayshortskip=8pt plus 4pt 
\belowdisplayskip=8pt plus 4pt minus 0pt 
\belowdisplayshortskip=8pt plus 4pt minus 0pt 

\floatsep 8pt plus 4pt minus 0pt 
\textfloatsep 8pt plus 4pt minus 0pt
\intextsep 8pt plus 2pt minus 1pt  
\dblfloatsep 16pt plus 4pt minus 0pt 
\dbltextfloatsep 16pt plus 4pt minus 0pt 

%\@fptop 6pt plus 4fil \@fpsep 6pt plus 4fil \@fpbot 6pt plus 4fil  \@dblfptop 8pt plus 4fil \@dblfpsep 8pt plus 4fil \@dblfpbot 8pt plus 4fil


\makeatother

\def\closemath{
\abovedisplayskip=3pt plus 3pt minus 1pt 
\abovedisplayshortskip=3pt plus 1pt minus 1pt 
\belowdisplayskip=3pt plus 3pt minus 1pt 
\belowdisplayshortskip=3pt plus 1pt minus 1pt }

\def\tightmath{
\abovedisplayskip=4pt plus 2pt minus 1pt 
\abovedisplayshortskip=4pt plus 1pt minus 1pt 
\belowdisplayskip=4pt plus 2pt minus 1pt 
\belowdisplayshortskip=4pt plus 1pt minus 1pt }
\def\crushmath{
\abovedisplayskip=1pt plus 1pt minus 2pt 
\abovedisplayshortskip=1pt plus 1pt minus 2pt 
\belowdisplayskip=1pt plus 1pt minus 2pt 
\belowdisplayshortskip=1pt plus 1pt minus 2pt }
\tightmath


==> tex-figs/DaliFaceBriar.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{assets/DaliFaceBriarv1.png}
    \vspace{-10pt}
    \caption{ROC and TAR@FAR of 1\%  for various recent face algorithms on the real long-distance   (RLD)) dataset. The improvement of  DaliFace over other prior state-of-the-art algorithms is more than the gaps between previous algorithms and is consistent with other experiments.}
    \label{fig:DaliFaceBriar}
\end{figure}


==> tex-figs/dali.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=.23\textwidth]{assets/persistence.jpg}
    \caption{A human can easily recognize distorted clocks in \emph{The Persistence of Memory}\footnotemark. In this light, we design a training procedure that learns representations that are invariant to real-world distortions, such as atmospheric turbulence.}
    \label{fig:dali}
\end{figure}

\footnotetext{todo add note on copyright}

==> tex-figs/weights_evolution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.25\textwidth]{assets/weights_evolution.png}
    \vspace{-10pt}
    \caption{Weights adaptation for each distortion level along the training epochs. Higher distortion levels (higher \textit{DL} values) start with lower weights which are progressively increased along the training until all of them reach the same value. All the weights are normalized between 0 and 1.}
    \label{fig:weights_evolution}
\end{figure}

